A Physics-Informed Vector Quantized Autoencoder for Data Compression of Turbulent Flow

Analyzing large-scale data from simulations of turbulent flows is memory intensive, requiring significant resources. This major challenge highlights the need for data compression techniques. In this study, we apply a physics-informed Deep Learning technique based on vector quantization to generate a discrete, low-dimensional representation of data from simulations of three-dimensional turbulent flows. The deep learning framework is composed of convolutional layers and incorporates physical constraints on the flow, such as preserving incompressibility and global statistical characteristics of the velocity gradients. The accuracy of the model is assessed using statistical, comparison-based similarity and physics-based metrics. The training data set is produced from Direct Numerical Simulation of an incompressible, statistically stationary, isotropic turbulent flow. The performance of this lossy data compression scheme is evaluated not only with unseen data from the stationary, isotropic turbulent flow, but also with data from decaying isotropic turbulence, and a Taylor-Green vortex flow. Defining the compression ratio (CR) as the ratio of original data size to the compressed one, the results show that our model based on vector quantization can offer CR $=85$ with a mean square error (MSE) of $O(10^{-3})$, and predictions that faithfully reproduce the statistics of the flow, except at the very smallest scales where there is some loss. Compared to the recent study based on a conventional autoencoder where compression is performed in a continuous space, our model improves the CR by more than $30$ percent, and reduces the MSE by an order of magnitude. Our compression model is an attractive solution for situations where fast, high quality and low-overhead encoding and decoding of large data are required.

==> Computational_Details.tex <==
% \subsection{Data}
% We train our model using high-fidelity DNS data of a three-dimensional, statistically stationary, isotropic turbulent flow with Taylor-Reynolds number $R_\lambda = 90$, solved on a cubic domain with $128$ grid points in each direction (DNS 1 in Table~\ref{tab:parameters}). More details on the DNS can be found in our previous works (\cite{ireland2013highly,momenifar2020local,momenifar2018influence}). In our training data set we have $40$ snapshots (as opposed to $3000$ in the recent study of \cite{glaws2020deep}) equally spaced in time, covering a time span of $2T_{l}$ ($T_{l}$ denotes large eddy turn over time). Each snapshot consists of the three components of the velocity field ($u , v, w$) at all $128^3$ grid points.

% We test the performance of the trained framework on a variety of flows to determine how well the model can compress flows different from those used in the training. For comparison purposes, the flows are selected to correspond to those considered in \cite{glaws2020deep}. Specifically, we start with statistically stationary isotropic turbulence, but then consider decaying isotropic turbulence, a Taylor-Green vortex flow, and finally a turbulent channel flow which possesses strong anisotropy and inhomogeneity (neither of which are present in the training data). The test snapshot of stationary isotropic turbulence comes from the same DNS that was used for training the model, but this snapshot is from a time that is $2T_{l}$ beyond the time of the last snapshot used in the training set. We obtained the snapshot for decaying isotropic turbulence from the Github repository of \cite{glaws2020deep}, which represents a flow with $R_\lambda = 89$ simulated on a $128^3$ grid. Our Taylor-Green vortex snapshot comes from a DNS with $Re = 1600$ (where $\nu = 1/1600$) performed on a $192^3$ grid, similar to that used in  \cite{glaws2020deep}. Finally, our channel flow snapshot comes from a DNS using a $2\pi \: \times 2 \: \times \pi$ domain with friction Reynolds number $Re_{\tau} = 180$, performed on a $128 \times 129 \times 128$ grid.


We train our model using high-fidelity DNS data of a three-dimensional, statistically stationary, isotropic turbulent flow with Taylor-Reynolds number $R_\lambda = 90$, solved on a cubic domain with $128$ grid points in each direction. More details on the DNS can be found in our previous works (\cite{ireland2013highly,momenifar2020local,momenifar2018influence}). In our training data set we have $40$ snapshots (as opposed to $3000$ in the recent study of \cite{glaws2020deep}) equally spaced in time, covering a time span of $2T_{l}$ ($T_{l}$ denotes large eddy turn over time). Each snapshot consists of the three components of the velocity field ($u , v, w$) at all $128^3$ grid points.

We test the performance of the trained framework on a variety of flows to determine how well the model can compress flows different from those used in the training. For comparison purposes, the flows are selected to correspond to those considered in \cite{glaws2020deep}. Specifically, we start with statistically stationary isotropic turbulence, but then consider decaying isotropic turbulence, a Taylor-Green vortex flow, and finally a turbulent channel flow which possesses strong anisotropy and inhomogeneity (\textit{neither of which are present in the training data}). The test snapshot of stationary isotropic turbulence comes from the same DNS that was used for training the model, but this snapshot is from a time that is $2T_{l}$ beyond the time of the last snapshot used in the training set. We obtained the snapshot for decaying isotropic turbulence from \cite{glaws2020deep}, which represents a flow with $R_\lambda = 89$ simulated on a $128^3$ grid. Our Taylor-Green vortex snapshot comes from a DNS with $Re = 1600$ (where $\nu = 1/1600$) performed on a $192^3$ grid, similar to that used in  \cite{glaws2020deep}. Finally, our channel flow snapshot comes from a DNS using a $2\pi \: \times 2 \: \times \pi$ domain with friction Reynolds number $Re_{\tau} = 180$, performed on a $128 \times 129 \times 128$ grid.



% \begin{comment}
% %\begin{tabular}{cc}
% 		$\mathrm{Parameter}$ & $\mathrm{DNS} \,1 $    \\
% 		$N$ & 128   \\
% 		$Re_\lambda$ &  93  \\
% 		$\mathscr{L}$ & 2$\upi$   \\       
% 		$\nu$ & 0.005  \\
% 		$\epsilon$ & 0.324 \\
% 		$l$ & 1.48  \\
% 		$l/\eta$ & 59.6  \\
% 		$u'$ & 0.984  \\
% 		$u'/u_\eta$ & 4.91  \\
% 		$T_L$ & 1.51  \\
% 		$T_L/\tau_\eta$ & 12.14  \\
% 		$\kappa_{{\rm max}}\eta$ & 1.5 \\
% %\end{tabular}
% \end{comment}


%
% \begin{table}[]
% \caption{Simulation parameters for the DNS study of isotropic turbulence (arbitrary units).
% $N$ is the number of grid points in each direction, 
% $Re_\lambda \equiv u'\lambda/\nu$ is the Taylor micro-scale Reynolds number ($Re_\lambda \equiv \sqrt{15Re}$ for homogeneous and isotropic flows), $\lambda\equiv u'/\langle(\boldsymbol{\nabla} \boldsymbol{u})^2\rangle^{1/2} $ is the Taylor micro-scale, $\mathscr{L} $ is the box size, $\nu$ is the fluid kinematic viscosity, $\epsilon \equiv 2\nu \int_0^{\kappa_{\rm max}}\kappa^2 E(\kappa) {\rm d}\kappa $ is the mean turbulent kinetic energy dissipation rate, $l \equiv 3\upi/(2k)\int_0^{\kappa_{\rm max}}E(\kappa)/\kappa {\rm d}\kappa $  is the integral length scale, $\eta \equiv \nu^{3/4}/\epsilon^{1/4}$ is the Kolmogorov length scale, $u' \equiv \sqrt{(2k/3)}$ is the fluid r.m.s. fluctuating velocity, $k$ is the turbulent kinetic energy, $u_\eta$ is the Kolmogorov velocity scale, 
% $T_L \equiv l/u^\prime$ is the large-eddy turnover time, $\tau_\eta \equiv \sqrt{(\nu/\epsilon)}$ is the Kolmogorov time scale, $\kappa_{\mathrm max}=\sqrt{2}N/3$ is the maximum resolved wavenumber.}
% {\begin{tabular}{cccccc}
% \hline
% $N$      & $Re_\lambda$ & L           & $\nu$ & $\epsilon$      & $l$                      \\ \hline
% 128      & 93           & 2$\upi$     & 0.005 & 0.324           & 1.48                     \\ \hline
% $l/\eta$ & $u'$         & $u'/u_\eta$ & $T_L$ & $T_L/\tau_\eta$ & $\kappa_{{\mathrm max}}\eta$ \\ \hline
% 59.6     & 0.984        & 4.91        & 1.51  & 12.14           & 1.5                      \\ \hline
% \end{tabular}}
% \label{tab:parameters}
% \end{table}

% \begin{table}[hbtp]
% \centering
% \label{tab:parameters}
% \caption{Simulation parameters for the DNS study of isotropic turbulence (arbitrary units).
% 		$N$ is the number of grid points in each direction, 
% 		$Re_\lambda \equiv u'\lambda/\nu$ is the Taylor micro-scale
% 		Reynolds number, $\lambda $ is the Taylor micro-scale,
% 		$\mathscr{L} $ is the box size, $\nu$ is the fluid kinematic viscosity, $\epsilon$ is the mean
% 		turbulent kinetic energy dissipation rate,
% 		$l$  is the integral length scale, $\eta \equiv \nu^{3/4}/\epsilon^{1/4}$ is the Kolmogorov length scale, 
% 		$u' \equiv \sqrt{(2k/3)}$ is the fluid r.m.s. fluctuating 
% 		velocity, $k$ is the turbulent kinetic energy, 
% 		$u_\eta$ is the Kolmogorov velocity scale, 
% 		$T_L \equiv l/u^\prime$ is the large-eddy turnover
% 		time, $\tau_\eta \equiv \sqrt{(\nu/\epsilon)}$ is the Kolmogorov time scale, 
% 		$\kappa_{\rm max}=\sqrt{2}N/3$ is the maximum resolved wavenumber.}
% % \resizebox{1\columnwidth}{!}{
% \begin{tabular}{@{}cc@{}}
% \toprule
% Parameter                & Value   \\ \midrule
% $N$                      & 128     \\
% $Re_\lambda$             & 93      \\
% $\mathscr{L} $           & 2$\upi$ \\
% $\nu$                    & 0.005   \\
% $\epsilon$               & 0.324   \\
% $l$                      & 1.48    \\
% $l/\eta$                 & 59.6    \\
% $u'$                     & 0.984   \\
% $u'/u_\eta$              & 4.91    \\
% $T_L$                    & 1.51    \\
% $T_L/\tau_\eta$          & 12.14   \\
% $\kappa_{{\rm max}}\eta$ & 1.5     \\ \bottomrule
% \end{tabular}
% % }
% \end{table}

%\FloatBarrier
%


\subsection{Model Hyper-Parameters}
As explained in the previous section, the VQ-AE network provides a compressed representation of data in a discrete/quantized latent space by vector-quantizing the intermediate representations of the autoencoder. Such discrete representations are more compact than the original data, while the reconstructed data has minimal distortion. We design our network so that it can transform and downsample original data by a scaling factor of $SF \in \{2,4,8\}$ depending on the level of reconstruction quality and compression needed. With $K = 512$ representing the size of the codebook (number of codewords) and mapping three velocity components into one in the discrete latent space, we can achieve $\frac{3 \times 32}{1 \times 9} \times (SF)^{3}$ reduction in bits, corresponding to $85$, $683$ and $5461$ when $SF$ is $2$, $4$ and $8$, respectively. Indeed, an input data of shape $(3,128,128,128)$ is compressed to $(1,64,64,64)$ with $SF=2$, $(1,32,32,32)$ with $SF=4$ or $(1,16,16,16)$ with $SF=8$.

We trained three versions of the model in which all of the hyper-parameters (of frameworks) are the same except the scaling factor, $SF$. 
Throughout our framework, each covolution layer is followed by a batch normalization (BN) layer and a rectified linear unit activation function, so called $ReLU$ ($ReLU(x)=max(0,x)$). Embedding batch normalization layer  \cite{ioffe2015batch} adjusts (scales to unit variance and zero mean) the intermediate outputs of each convolutional layer so that their distributions are more stable throughout the framework. This batch normalization layer is frequently used in the deep learning community and is known to accelerate the training of deep neural nets.

We use three types of convolutional layers, type 1 with kernel size $4$ and stride length $2$ (used for the purpose of dimension reduction/expansion), type 2 with kernel size $3$ and stride length $1$ and type 3 with kernel size $1$ and stride length $1$ for learning transformation. The number of convolutional layers in their networks depends on the scaling factor $SF$. When $SF=2$, the encoder is composed of one type 1 kernel followed by a type 2 kernel, while the decoder consists only of one type 1 kernel. Similarly with $SF=8$, the encoder is composed of three type 1 kernels followed by one type 2 kernel, while the decoder has three type 1 kernels. We also use residual blocks (\cite{he2016deep}) to obtain a robust performance as the networks become deeper, without which there could arise optimization issues due to vanishing/exploding gradients. We embedded only 2 residual blocks, as opposed to 12 in \cite{glaws2020deep}, where each block is composed of two type 2 kernels convolutional layers which are embedded at the end of encoder and the beginning of decoder networks. Such a framework drastically reduces the number of learnable parameters compared to the recent fully convolutional autoencoder in \cite{glaws2020deep}. The schematic of this framework is shown in figure \ref{fig:VQ-AE_Schematic}.

%
% \begin{figure}
% 	\centering	
% 	\includegraphics[width=1\linewidth]{./Fig1.pdf}
% 	\caption{Schematic of the VQ-AE architecture. In this figure, $N$ is the number of training data in a batch of them, $C$ is the number of channels in the input data (corresponding with the number of velocity components), $H$ , $W$ and $D$ represent the height, width and depth of input data, and $SF \in \{2,4,8\}$ is the scaling factor.}
% 	\label{fig:VQ-AE_Schematic}
% \end{figure}
%\FloatBarrier
%

We designed a codebook with $K = 512$ codewords, each with embedding dimension $64$. For the loss function hyper-parameters, we use commitment loss coefficient $\beta = 0.25$ (as suggested in \cite{van2017neural}), $\alpha = 0.1$ and $a = 2$ for the velocity gradient constraint (motivated by the knowledge that at the small-scales of isotropic turbulence, the variance of the transverse velocity gradients are twice the size of the longitudinal ones \cite{pope_2000}), and finally $\gamma = 10^{-4}$ for the term corresponding to other constraints. It is worth mentioning that an improved reconstruction of the velocity gradient tensor would eventually lead to better results for the terms in the other constraint, which is the reason for setting $\alpha \gg \gamma$. We trained our framework for 200 epochs with batch size $=1$ using the Adam optimizer \cite{kingma2014adam} with learning rate = $0.001$, along with a learning rate scheduler. 
It should be noted that our focus has been on the general characteristics of the framework rather than achieving the best configurations, hence there might be room for improvements by tuning the proposed hyper-parameters. 
We implemented this framework in PyTorch using the CUDA environment, and trained it on one NVIDIA Pascal P100 GPU. The training was completed within approximately 8 hours, and the maximum GPU memory consumed was around 5 $GB$.


%hidden size (number of channels) of residual blocks = 32

==> Evaluation_Metrics.tex <==

In addition to the conventional error measurement methods such as MSE and mean absolute error (MAE), the performance of the reconstructed field is assessed using additional diagnostic tests from the image processing community, as well as rigorous physics-based metrics relevant to the analysis of turbulence.
We employ two image similarity metrics (i) the peak signal-to-noise-ratio (PSNR) defined as

\begin{eqnarray}\label{eq:PSNR}
 PSNR (x,\hat{x}) = 10 \: log_{10} \Big(\frac{MAX(x,\hat{x})^{2}}{MSE(x,\hat{x})}\Big)
\end{eqnarray}
which, unlike the MSE, can handle grid data with different dynamic ranges,
and (ii) the mean structural similarity index measure (MSSIM) \cite{wang2004image}. For brevity, we do not repeat the concept or equations related to the MSSIM metric as it is already well explained in the recent study of \cite{glaws2020deep}. 

For the physics-based quality metrics, in addition to the already defined Betchov relations, we consider the turbulence kinetic energy spectra, and the probability density functions (PDFs) of the filtered velocity gradient tensor and its invariants. The turbulent kinetic energy spectra provides information on the kinetic energy content at different scales in the flow, providing crucial quantitative information on the flow. However, the energy spectrum does not provide information on the rich, multiscale statistical geometry in the flow which is crucial for the dynamics of turbulence, nor does it provide information on intermittent fluctuations in the flow. For example, the geometric alignments between the strain-rate and vorticity fields play an important role in the fundamental process of vortex stretching which in turn is crucial for the generation of intermittent fluctuations in the flow \cite{buaria20}, and these small scales processes in turbulence are captured by analyzing the velocity gradient tensor $\boldsymbol{A}$ \cite{tsinober,meneveau11}. Moreover, by filtering $\boldsymbol{A}$ at different scales to obtain the filtered velocity gradient tensor, $\widetilde{\boldsymbol{A}}$, one can analyze the multiscale properties of the flow and processes such as the energy cascade \cite{danish18,carbone20,johnson20,tom21}. Therefore, to provide a more thorough test of the quality of the reconstructed fields, in addition to the energy spectrum we also consider PDFs of the diagonal and off-diagonal components of $\widetilde{\boldsymbol{A}}$, as well as joint PDFs of the principal invariants of $\widetilde{\boldsymbol{A}}$, namely $Q\equiv-\frac{1}{2}tr(\widetilde{\boldsymbol{A}}^2)$ and $R\equiv-\frac{1}{2}tr(\widetilde{\boldsymbol{A}}^3)$. The joint PDF of $Q,R$ provides rich information and is commonly used to assess the basic properties of turbulent flows \cite{tsinober,meneveau11}, with $Q$ measuring the relative importance of strain and rotation rates at a point in the flow ($Q > 0$ indicates rotation dominated regions), while $R$ measures the relative importance of strain self-amplification (SSA) and vortex stretching (VS) at a point in the 
flow ($R > 0$ indicates SSA dominated region). In our results, to construct $\widetilde{\boldsymbol{A}}$ we convolve $\boldsymbol{A}$ with a low-pass Gaussian filter for three different filtering lengths, corresponding to filtering in the dissipation, inertial, and large scale (energy containing) ranges of the turbulent flow.








==> Makefile <==
FILENAME = dcc_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

